DialogGen: Multi-modal Interactive Dialogue System for Multi-turn Text-to-Image Generation

Text-to-image (T2I) generation models have significantly advanced in recent years. However, effective interaction with these models is challenging for average users due to the need for specialized prompt engineering knowledge and the inability to perform multi-turn image generation, hindering a dynamic and iterative creation process. Recent attempts have tried to equip Multi-modal Large Language Models (MLLMs) with T2I models to bring the user's natural language instructions into reality. Hence, the output modality of MLLMs is extended, and the multi-turn generation quality of T2I models is enhanced thanks to the strong multi-modal comprehension ability of MLLMs. However, many of these works face challenges in identifying correct output modalities and generating coherent images accordingly as the number of output modalities increases and the conversations go deeper. Therefore, we propose DialogGen, an effective pipeline to align off-the-shelf MLLMs and T2I models to build a Multi-modal Interactive Dialogue System (MIDS) for multi-turn Text-to-Image generation. It is composed of drawing prompt alignment, careful training data curation, and error correction. Moreover, as the field of MIDS flourishes, comprehensive benchmarks are urgently needed to evaluate MIDS fairly in terms of output modality correctness and multi-modal output coherence. To address this issue, we introduce the Multi-modal Dialogue Benchmark (DialogBen), a comprehensive bilingual benchmark designed to assess the ability of MLLMs to generate accurate and coherent multi-modal content that supports image editing. It contains two evaluation metrics to measure the model's ability to switch modalities and the coherence of the output images. Our extensive experiments on DialogBen and user study demonstrate the effectiveness of DialogGen compared with other State-of-the-Art models.

==> tabs/correction_example.tex <==
\begin{exmp}{Correction examples}{correction_eg}
    \small
    \textbf{History:} (empty)\\
    \textbf{Question:} I'd like to know more about rockets. Could you draw me a picture of rockets?\\
    \textbf{Original Output:}\textless{}draw\textgreater{}A rocket is a large, powerful, and complex machine that is used to transport people and goods into space. It is usually made of steel and aluminum and is equipped with engines, fuel tanks, guidance systems, and other equipment. The picture shows a large rocket with a long tail, flying high in the sky.\\
    \textbf{Correction:} The output violates rule 3. The assistant's description misses the main points of the asking for a visual image of a rocket.\\
    \textbf{Correct Solution:}\textless{}draw\textgreater{}A rocket propelled upward by burning flames is moving through space, the Milky Way and stars in the background, the shot is panoramic, and the style is cartoonish.\\

\end{exmp}

==> tabs/correction_exps1.tex <==
% \begin{table*}[t]
% % \renewcommand\arraystretch{0.8}
% % \Huge
% \caption{Comparison of Modality Switching (MS) ability and Drawing Instruction Following (DIF) of different models under standard fine-tuning and error correction counterparts with different style .
% }
% \label{tab:correction_exps1}
% \centering
% % \resizebox{.99\linewidth}{!}{
% \begin{tabular}{@{}clccccc@{}}
% \toprule
% \multirow{2}{*}{Model} & \multicolumn{1}{c}{\multirow{2}{*}{Training}} & \multirow{2}{*}{\#Inference}& \multicolumn{2}{c}{DialogBen-MS} &\multicolumn{2}{c}{DialogBen-DIF} &   \cmidrule(l){4-7} 
%  & \multicolumn{1}{c}{} &  & 1st / 2nd / 3rd & Avg. & 1st / 2nd / 3rd & Avg. \\ \midrule
% \multirow{3}{*}{DialogGen-baseline} & Standard Fine-Tuning & 1-step &  93.6 / 87.1 / 84.6 & 88.4 & 97.3 / 96.3 / 95.0 & 96.2  \\
%  & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}1-step & \cellcolor{purple1!25}96.9 / 95.6 / 93.4 & \cellcolor{purple1!25}95.3(+6.9) & \cellcolor{purple1!25} 98.0 / 96.9 / 96.2 & 97.0(+0.8) \cellcolor{purple1!25}  \\
%   & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}2-step & \cellcolor{purple1!25} 97.8 / 97.4 / 93.6 & \cellcolor{purple1!25}96.2(+7.8) & \cellcolor{purple1!25} -   & \cellcolor{purple1!25} - \\ \midrule
% \multirow{3}{*}{DialogBen} & Standard Fine-Tuning & 1-step & 96.4 / 96.5 / 95.6 &  96.1\\
%  & \cellcolor{purple1!25} + Error Correction  &  \cellcolor{purple1!25}1-step & \cellcolor{purple1!25}97.1 / 97.9 / 96.7  & \cellcolor{purple1!25} 97.2 (+1.1) & \cellcolor{purple1!25} & \cellcolor{purple1!25} \\
%  & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}2-step & \cellcolor{purple1!25} 97.3 / 97.9 / 96.9 &   \cellcolor{purple1!25}97.4 (+1.3) & \cellcolor{purple1!25} & \cellcolor{purple1!25} 
%  \\ \bottomrule
% \end{tabular}
% % }
% \end{table*}



==> tabs/merge_correction_exps_multilingual.tex <==
% \begin{minipage}{\textwidth}

% \begin{minipage}[t]{0.48\textwidth}
% \makeatletter\def\@captype{table}
% \begin{table*}[t]
% % \renewcommand\arraystretch{0.8}
% % \Huge
% \caption{Comparison of Modality Switching (MS) ability  of different models under standard fine-tuning and error correction counterparts with different style .
% }
% \label{tab:correction_exps}
% \centering
% \resizebox{.8\linewidth}{!}{
% \begin{tabular}{@{}clccc@{}}
% \toprule
% \multirow{2}{*}{Model} & \multicolumn{1}{c}{\multirow{2}{*}{Training}} & \multirow{2}{*}{\#Inference}& \multicolumn{2}{c}{DialogBen-MS} 
%  & \multicolumn{3}{c}{}  & 1st / 2nd / 3rd & Avg.  \\ \midrule
% \multirow{3}{*}{DialogGen-A} & Standard Fine-Tuning & 1-step &  93.6 / 87.1 / 84.6 & 88.4   \\
%  & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}1-step & \cellcolor{purple1!25}96.9 / 95.6 / 93.4 & \cellcolor{purple1!25}95.3(+6.9)    \\
%   & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}2-step & \cellcolor{purple1!25} 97.8 / 97.4 / 93.6 & \cellcolor{purple1!25}96.2(+7.8)  \\ \midrule
% \multirow{3}{*}{DialogBen} & Standard Fine-Tuning & 1-step & 96.4 / 96.5 / 95.6 &  96.1\\
%  & \cellcolor{purple1!25} + Error Correction  &  \cellcolor{purple1!25}1-step & \cellcolor{purple1!25}97.1 / 97.9 / 96.7  & \cellcolor{purple1!25} 97.2 (+1.1)  \\
%  & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}2-step & \cellcolor{purple1!25} 97.3 / 97.9 / 96.9 &   \cellcolor{purple1!25}97.4 (+1.3)  
%  \\ \bottomrule
% \end{tabular}
% }
% \end{table*}
% \end{minipage}

% \begin{minipage}[t]{0.48\textwidth}
% \makeatletter\def\@captype{table}
% \begin{table*}[t]
% % \renewcommand\arraystretch{0.8}
% % \Huge
% \caption{Comparison of adding bilingual training on Modality Switching Accuracy.
% }
% \label{tab:multilingual}
% \centering
% \resizebox{.99\linewidth}{!}{
% \begin{tabular}{@{}clccccc@{}}
% \toprule
% \multirow{2}{*}{Model} & \multicolumn{1}{c}{\multirow{2}{*}{Training}} & \multicolumn{1}{c}{\multirow{2}{*}{Evaluation Data}} & \multicolumn{4}{c}{DialogBen-MS}  &   \cmidrule(l){4-7} 
%  & \multicolumn{1}{c}{} &  & Round1 & Round2 & Round3 & Avg  \\ \midrule
% \multirow{2}{*}{Qwen-VL} & DialogBen-train-en &DialogBen-test-en  & 77.8 / 97.6 / 97.0 / 95.6 & 77.5 / 98.4 / 96.2 / 88.7 & 79.9 / 95.6 / 95.7 / 79.6 & 90.0  \\
%  & \cellcolor{purple1!25} + DialogBen-train-cn & DialogBen-test-en  & \cellcolor{purple1!25}78.2 / 96.9 / 97.0 / 96.0 & \cellcolor{purple1!25}83.0 / 97.6 / 96.6 / 89.5 & \cellcolor{purple1!25}82.5 / 96.7 / 95.4 / 85.4 & \cellcolor{purple1!25}91.3 (+1.3)  \\ \midrule
% \multirow{2}{*}{Qwen-VL} & DialogBen-train-cn  & DialogBen-test-cn  & 82.5 / 98.0 / 97.0 / 97.0 & 76.0 / 99.0 / 94.0 /92.0 & 71.0 / 97.9 / 93.6 / 83.8 & 90.1  \\
%  & \cellcolor{purple1!25} + DialogBen-train-en & DialogBen-test-cn   & \cellcolor{purple1!25}87.0 / 98.4 / 97.7 / 98.7 & \cellcolor{purple1!25}90.4 / 99.2 / 95.3 / 95.0 & \cellcolor{purple1!25}86.0 / 98.0 / 92.6 / 89.2 & \cellcolor{purple1!25}94.0(+3.9)  
%  \\ \bottomrule
% \end{tabular}
% }
% \end{table*}
% \end{minipage}
% \end{minipage}




\noindent
\begin{minipage}{\textwidth}
% \captionof{}{xxxx}
\begin{minipage}[t]{0.48\textwidth}
    \captionof{table}{Comparison of Modality Switching (MS) accuracy (\%) of different models under standard fine-tuning and error correction counterparts with different inference styles.}
    \label{tab:correction_exps}
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}clccc@{}}
        \toprule
        {Model} & \multicolumn{1}{c}{{Training}} & {\#Inference} & {DialogBen-MS Avg.} \\
        \midrule
        \multirow{3}{*}{DialogGen-A} & Standard Fine-Tuning & 1-step & 88.4   \\
        & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}1-step & \cellcolor{purple1!25}95.3(+6.9)    \\
        & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}2-step  & \cellcolor{purple1!25}96.2(+7.8)  \\
        \bottomrule
        \multirow{3}{*}{DialogBen} & Standard Fine-Tuning & 1-step &  96.1\\
 & \cellcolor{purple1!25} + Error Correction  &  \cellcolor{purple1!25}1-step & \cellcolor{purple1!25} 97.2 (+1.1)  \\
 & \cellcolor{purple1!25} + Error Correction & \cellcolor{purple1!25}2-step  &   \cellcolor{purple1!25}97.4 (+1.3)  
 \\ \bottomrule
        \end{tabular}
    }
\end{minipage}%
\hfill
\begin{minipage}[t]{0.48\textwidth}
    \captionof{table}{Comparison of adding bilingual training on Modality Switching (MS) Accuracy (\%) of models under different training data. `cn' and `en' represent Chinese and English data respectively.} 
    \label{tab:multilingual}
    \centering
    % \vspace{7.8mm}
    \resizebox{.99\linewidth}{!}{
        \begin{tabular}{@{}ccccccc@{}}
        \toprule
        {Model} & \multicolumn{1}{c}{{Training}} & \multicolumn{1}{c}{Evaluation} & {DialogBen-MS Avg.} \\
        \midrule
        \multirow{2}{*}{Qwen-VL} & en & en & 90.0  \\
        & \cellcolor{purple1!25} bilingual & en & \cellcolor{purple1!25}91.3 (+1.3)  \\
        \midrule
\multirow{2}{*}{Qwen-VL} & cn  & cn  & 90.1  \\
 & \cellcolor{purple1!25} bilingual & cn   & \cellcolor{purple1!25}94.0(+3.9)  
 \\ \bottomrule
        \end{tabular}
    }
\end{minipage}
\end{minipage}


==> tabs/prompt_drawing_instruction_following.tex <==
\begin{exmp}{Prompt For Drawing Instruction Following}{following_prompt}
\label{prompt for drawing instruction following}
    \small

    You are an expert who performs judgment on the output results of the multi-modal large language model AI that supports the three-turn dialogue drawing function:
    
1. The input may contain images. It is especially identified by \textless{}img\textgreater{} and \textless{}/img\textgreater{}  where the detailed description of the image lies between them.

2. For the input of a user, it will first identify whether the intention of the user is to draw or talk, if it is to draw it will append \textless{}draw\textgreater{} before the output.

3. If the user's intention is to talk, then the output of the assistant in the current turn should be coherent in response to the user query.

4. If the user's intention is to draw, then the output of the assistant in the current turn should be \textless{}draw\textgreater{} and a detailed description prompt in response to the user's need. The prompt should be able to be directly sent into the image generation model to produce high-quality images.

You need to perform correctness judgment on the results of the current dialogue output of the AI. For each round of dialogue, the input is "historical dialogue" and "current request", and the output is "drawing text". It is necessary to make the following judgments on the current output results: 

1. Determine whether the text content is indeed drawing text.

2. Determine whether the drawing text is detailed enough to meet the requirements of a generation model to generate the corresponding image.

3. Determine whether the output has irregular sentences, too many words, or too few words.

4. Determine whether the dialogue meets the 3 requirements of the three rounds of dialogue content and format instructions.

Only the current output needs to be judged, and errors in historical conversations are not considered. If the judgment of the current output result is that the above nine conditions are all yes, then output "\#\#\#Correct", if not sure, output "\#\#\#Uncertain", otherwise output "\#\#\#Wrong" and explain what should be done. Modify to make the output meet the requirements, separated by '\#\#\#':\\
    (3 in-context examples)\\
    \textbf{Historical dialogue:} $q_{i}$\\
    \textbf{Current Request:} $r_{i}$\\
    \textbf{Output:} \{Completion\} \\
    \textbf{Perform correctness judgment:}

\end{exmp}

==> tabs/prompt_example_v2.tex <==
\begin{exmp}{Prompt For Generating Corrections}{correction_prompt}
\label{prompt for error correction}
    \small

    
You are given the history conversation H, user query in current turn Q, output of the assistant in current turn $R_{pre}$ and a suitable output given by human expert $R_{gt}$. 

You need to make the judgements as following rules:

1. According to the history and the current user query, make judgements on whether the model correctly identifies the use's intention.

2. If the intention of the user is to talk, make judgements on whether the output of the assistant following the instructions of the user coherently.

3. If the intention of the user is to draw, make judgements on whether the output prompt is indeed a descriptive text that is suitable for a image generation model to generate images.

If the output satisfy all the three criteria, output '\#\#\#Correct'. If not, output '\#\#\#Wrong\#\#\#' and the specific criteria it violates followed by an explanation and provide a correct output for current user query..\\
    
    % \textbf{Question:} \\
    % \textbf{Original Output:}\\
    % xxxxxxxxx\\
    % \textbf{Correction:} ......\\
    % \textbf{Correct Solution:}\\
    % ...\\

    (3 in-context examples)\\

    \textbf{Question:} $q_{i}$\\
    \textbf{Original Output:} $r_{i}$\\
    \textbf{Correction:} \{Completion\}

\end{exmp}

You are an expert in providing feedback on the output of an Multi-modal Large Language Model that supports multi-turn multi-modal dialog and image generation, the behaviour of the assitant is listed as follows:
1. The input may contains images. It is specailly identified by <img> and </img> where the detailed description of the image lies between them.
2. For the input of an user, it will first identify the whether the intention of the user is draw or talk, if it is to draw it will append '<draw>' before the output.
3. If the user intention is to talk, then the output of the assistant in current turn should be coherent in response to the user query.
4. If the user intention is to draw, then the output of the assistant in current turn should be '<draw>' and a detailed description prompt in response to the user's need. The prompt should be able to be directly sent into the image generation model to produce high quality image.

You are given the history conversation H, user query in current turn Q, output of the assistant in current turn R_pre and a suitable output given by human expert R_gt. You need to make the judgements as following rules:
1. According to the history and the current user query, make judgements on whether the model correctly identifies the use's intention.
2. If the intention of the user is to talk, make judgements on whether the output of the assistant following the instructions of the user coherently.
3. If the intention of the user is to draw, make judgements on whether the output prompt follows the user's instruction and is indeed a descriptive text that is suitable for a image generation model to generate images.

If the output satisfy all the three criteria, output '###Correct'. If not, output '###Wrong###' and the specific criteria it violates followed by an explanation and provide a correct output for current user query.

You are given the following samples.
Sample1:
For H:{}, Q:{}, R_pre:{}, provide your feedback:
###wrong
###explanation:{}
###the suitable output should be like {}\n
Sample2:
For H:{}, Q:{}, R_pre:{}, provide your feedback:
###wrong
###explanation:{}
###the suitable output should be like {}\n
Sample3:
For H:{}, Q:{}, R_pre:{}, provide your feedback:
###wrong
###explanation:{} 
###the suitable output should be like {}\n

Now given H:{}, Q:{}, R_pre:{}, provide your feedback:

==> tabs/vqa_example.tex <==
\begin{exmp}{Coherence VQA}{vqa}
    \small
    % \tiny
    
    % History:\\
    \textbf{User}: \quad \quad \quad 
    {\includegraphics[width=0.3\textwidth]{images/kitchen.pdf}\\What kind of merchandise is this and what is it used for?
    \\
    \textbf{Assistant}: This product is an oven, mainly used for baking or roasting food, with temperature control and timing functions, is a common appliance in modern home kitchens.\\
    \textbf{User}: What if you change the color of the oven so that it fits more in with the kitchen decor, say silver? \\
    \textbf{Questions: } \\
    1. Is there an oven in the picture? \\
    2. Is the oven placed in the middle of a kitchen? \\
    3. Is the background of the picture a modern kitchen?\\
    4. Is the shot of this picture panoramic? \\
    5. Is the color of the oven in the picture silver? \\
}

\end{exmp}
